Tight Bounds on the Round Complexity of the Distributed Maximum Coverage Problem

We study the maximum $k$-set coverage problem in the following distributed setting. A collection of sets $S_1,\ldots,S_m$ over a universe $[n]$ is partitioned across $p$ machines and the goal is to find $k$ sets whose union covers the most number of elements. The computation proceeds in synchronous rounds. In each round, all machines simultaneously send a message to a central coordinator who then communicates back to all machines a summary to guide the computation for the next round. At the end, the coordinator outputs the answer. The main measures of efficiency in this setting are the approximation ratio of the returned solution, the communication cost of each machine, and the number of rounds of computation. Our main result is an asymptotically tight bound on the tradeoff between these measures for the distributed maximum coverage problem. We first show that any $r$-round protocol for this problem either incurs a communication cost of $ k \cdot m^{\Omega(1/r)}$ or only achieves an approximation factor of $k^{\Omega(1/r)}$. This implies that any protocol that simultaneously achieves good approximation ratio ($O(1)$ approximation) and good communication cost ($\widetilde{O}(n)$ communication per machine), essentially requires logarithmic (in $k$) number of rounds. We complement our lower bound result by showing that there exist an $r$-round protocol that achieves an $\frac{e}{e-1}$-approximation (essentially best possible) with a communication cost of $k \cdot m^{O(1/r)}$ as well as an $r$-round protocol that achieves a $k^{O(1/r)}$-approximation with only $\widetilde{O}(n)$ communication per each machine (essentially best possible). We further use our results in this distributed setting to obtain new bounds for the maximum coverage problem in two other main models of computation for massive datasets, namely, the dynamic streaming model and the MapReduce model.

==> communication.tex <==
\section{Communication Complexity Model}\label{app:communication} 

We prove our lower bound for distributed protocols using the framework of communication complexity, and in particular in the (number-in-hand) multiparty communication model
with shared blackboard: there are $p$ players (corresponding to machines) receiving inputs $(x_1,\ldots,x_p)$ from a prior distribution $\dist$ on $\XX_1 \times \ldots \XX_p$. 
The communication happens in rounds and in each round, the players \emph{simultaneously} write a message to a \emph{shared blackboard} visible to all parties. The message sent
by any player $i$ in each round can only depend on the input of the player, i.e., $x_i$, the current content of the blackboard, i.e., the messages communicated in previous rounds, and
public and private randomness. In addition to $p$ players, there exists a central party called the referee (corresponding to the coordinator) who only sees the content of the blackboard and public randomness and is 
responsible for outputting the answer in the final round. 

For a protocol $\prot$, we use $\Prot = (\Prot_1,\ldots,\Prot_p)$ to denote the transcript of the messages communicated by all players, i.e., the content of the blackboard. 
The \emph{communication cost} of a protocol $\prot$, denoted by $\norm{\prot}$, is the sum of worst-case length of the messages communicated by all players, i.e., $\norm{\prot} := \sum_{i=1}^{p} \card{\Prot_i}$. 
We further refer to $\max_{i \in [p]} \card{\Prot_i}$ as the \emph{per-player communication cost} of $\prot$. We remark that this model is identical to the distributed setting introduced earlier if we allow the coordinator to communicate with machines free of charge. As a result, communication lower bounds in this model
imply identical communication lower bounds for distributed protocols. We refer the reader to the excellent text by Kushilevitz and Nisan~\cite{KN97} for more details on communication complexity.



==> submodular.tex <==
\section{Submodular Maximization with Cardinality Constraint}\label{app:submodular}

Let $V = \set{a_1,\ldots,a_m}$ be a ground set of $m$ items. For any set function $f: 2^V \rightarrow \IR$ and any $A \subseteq V$, we define 
the \emph{marginal contribution} to $f$ as a set function $f_A: 2^{V} \rightarrow \IR$ such that for all $B \subseteq V$, $f_A(B) = f(A \cup B) - f(A)$. 
When clear from the context, we abuse the notation and for $a \in V$, use $f(a)$ and $f_A(a)$ instead of $f(\set{a})$ and $f_A(\set{a})$, respectively. 
A function $f$ is \emph{submodular} iff for all $A \subseteq B \subseteq V$ and for all $a \in V$, $f_B(a) \leq f_A(a)$. 
A submodular function $f$ is additionally \emph{monotone} iff $\forall A \subseteq B \subseteq V$, $f(A) \leq f(B)$. 

The maximum coverage problem is a special case of {maximizing a monotone submodular function} subject to a cardinality
constraint of $k$, i.e., finding $\Astar \in \argmax_{A: \card{A} = k} f(A)$: for any set $S$ in maximum coverage we can have an item $a_S \in V$ and 
for each $A \subseteq V$, define $f(A) = \card{\bigcup_{a_S \in A} S}$. It is easy to verify that $f(\cdot)$ is monotone submodular. 

We use the following standard facts about monotone submodular functions in our proofs. 

\begin{fact}\label{fact:submodular-greedy}
	Let $f(\cdot)$ be a monotone submodular function, then: 
	\begin{align*}
		\forall A \subseteq V, B \subseteq V ~~ f(B) \leq f(A) + \sum_{a \in B \setminus A} f_A(a). 
	\end{align*}
\end{fact}

\begin{fact}\label{fact:submodular-subadditive}
	Let $f(\cdot)$ be a submodular function, then, for any $A \subseteq V$, $f_A(\cdot)$ is subadditive, i.e., $f_A(B \cup C) \leq f_A(B) + f_A(C)$ for all $B,C \subseteq V$. 
\end{fact}

